STanH : Parametric Quantization for Variable Rate Learned Image Compression

In end-to-end learned image compression, encoder and decoder are jointly trained to minimize a $R + {\lambda}D$ cost function, where ${\lambda}$ controls the trade-off between rate of the quantized latent representation and image quality. Unfortunately, a distinct encoder-decoder pair with millions of parameters must be trained for each ${\lambda}$, hence the need to switch encoders and to store multiple encoders and decoders on the user device for every target rate. This paper proposes to exploit a differentiable quantizer designed around a parametric sum of hyperbolic tangents, called STanH , that relaxes the step-wise quantization function. STanH is implemented as a differentiable activation layer with learnable quantization parameters that can be plugged into a pre-trained fixed rate model and refined to achieve different target bitrates. Experimental results show that our method enables variable rate coding with comparable efficiency to the state-of-the-art, yet with significant savings in terms of ease of deployment, training time, and storage costs

==> chapters/4_experiments/6_quantizer_analysis.tex <==
\begin{figure}[h!]
%\begin{minipage}[b]{1.0\linewidth} 
  \centering
 \includegraphics[width=\columnwidth]{images/4_experiments/levels/Different_levels_zou.pdf}
 % \vspace{0.1cm}
  \caption{Distribution of Length of the quantization intervals for different qualities, taking \emph{Zou22} as Reference, considering derivations obtained from the highest rate anchor $A_{1}$}%\attilio{Possiamo girare questa figura di 90 gradi in senso antiorario ? Messa cisì, sembra che la variabile dipendente sia la width del quantization step piuttosto che l indice di quantizzazione}} 
  \label{anchor}
%\end{minipage}
\end{figure}



\subsection{Analysis of STanH quantizer} \label{functioning} 

%AF Questa parte sotto l'abbiamo già detta: è poco informativa e prende spazio e tempo di lettura al reviewer
%The idea behind the \stanh module is quite straightforward: maintain the same autoencoder for extracting useful compressed features while varying the quantization levels to regulate the desired level of quality.
%In this way, starting from the latent representation with the highest bitrates, it is possible to reduce the compression rate by slightly modifying the quantization procedure.
%In particular, 
Fig.~\ref{anchor} shows the width of the central quantization levels related to $\mathbf{\hat{y}}$ formed during training for \emph{Zou22} taking $A_{1}$ as anchor and three corresponding derivations ($D_{11},D_{12},D_{13}$), \alberto{whose performance are shown in the top-right corner of Fig.~\ref{2a}}.
We show only central quantization levels because they contain most of the information and vary the most between the anchor and the derivations.
On the vertical axis, there are the different quantization intervals considered, while on the horizontal one there are their length for different models;
The major differences are visible on the central levels, namely zero and one, 
where the lowest quality model has longer quantization intervals: almost doubling their length for the lowest quality ones. 
%\attilio{Sarebbe possibile in Fig 2 far vedere per beta -> inf esattamente questo caso, in modo che questa figura quantifichi i dettagli di Fig 2 ?}
From the figure, it is understood how, when one aims to optimize \stanh at a lower quality, both levels zero and one become progressively larger, thus encompassing more values during the quantization process and making it less refined.
\attilio{Se penso alla DCT mi viene da pensare ai coefficienti ad alta frequenza e il ragionamento non mi sembra sbagliato, però manca una conclusione a cui portare il lettore: cosa vogliamo verificare con questo grafico ?}






